Control and Placement of Finite-Resolution Intelligent Surfaces in IoT Systems with Imperfect CSI

In this paper, we study the advantages of using reconfigurable intelligent surfaces (RISs) for interference suppression in single-input single-output (SISO) distributed Internet of Things (IoT) networks. Implementing RIS-assisted networks confronts various problems, mostly related to the control and placement of the RIS. To tackle the control-related challenges, we consider noisy and local channel knowledge, based on which we devise algorithms to optimize the potentially distributed RISs to achieve an overall network objective, such as the sum-rate. We use a network with a centralized RIS as a benchmark for our comparisons. We further assume low-bit phase shifters at the RIS to capture real-world hardware limitations. We also study the placement of the RIS and analytically quantify the minimum required degrees-of-control for the RIS as a function of its location to guarantee a specific network performance metric and verify the results via simulations.

==> sections/Appendices_full_descrip.tex <==
\section{Proof of Lemma~\ref{lemma:approx_prob}}

\label{appndx:proof_approx_prob}

\begin{proof}
For a given $\mathbf{\Theta}$, we have
\begin{align}
\label{eq:intersect_real_imag}
    &\Pr\Big(\Big|\textbf{g}^{[i]}\mathbf{\Theta}\textbf{h}^{[j]}+h_d^{[ji]}\Big|<\delta\Big|\mathbf{\Theta}\Big) \\ \nonumber
    & \quad \quad \quad \quad >\Pr\Big(\Big|Re\{\textbf{g}^{[i]}\mathbf{\Theta}\textbf{h}^{[j]}+h_d^{[ji]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta} \bigcap \Big|Im\{\textbf{g}^{[i]}\mathbf{\Theta}\textbf{h}^{[j]}+h_d^{[ji]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta}\Big).
\end{align}
We define $X\triangleq Re\{\textbf{g}^{[i]}\mathbf{\Theta}\textbf{h}^{[j]}+h_d^{[ji]}\}$ and $Y\triangleq Im\{\textbf{g}^{[i]}\mathbf{\Theta}\textbf{h}^{[j]}+h_d^{[ji]}\}$ to make the proof easier to understand. Then, to simplify \eqref{eq:intersect_real_imag}, we need to show that $|X|$ and $|Y|$ are independent. We note that the independence of $X$ and $Y$ leads to the independence of $|X|$ and $|Y|$ since applying any function to two independent variables does not change the independence property. Thus, we remove the absolute function from the rest of the proof. Furthermore, from Lemma~\ref{lemma:avg_variance}, we know that $X$ and $Y$ are two random variables, which are distributed based on zero-mean Gaussian distribution. Therefore, $X$ and $Y$ are independent if they are uncorrelated (i.e., $Cov(X,Y)=0$). Hence, to show $Cov(X,Y)$, we write
\begin{align}
    Cov(X,Y)=\mathbb{E}(XY)-\mathbb{E}(X)\mathbb{E}(Y)\overset{(a)}{=}\mathbb{E}(XY),
\end{align}
where $(a)$ holds because $X$ and $Y$ are zero-mean random variables. Then, we have
\begin{align}
\label{eq:e_xy_ini}
    \mathbb{E}(XY)=\mathbb{E}\Big\{Re\{\sum_{m=1}^Mg_{m}^{[i]}e^{j\theta_m}h_{m}^{[j]}+h_d^{[ji]}\}Im\{\sum_{m^{\prime}=1}^Mg_{m^{\prime}}^{[i]}e^{j\theta_{m^{\prime}}}h_{m^{\prime}}^{[j]}+h_d^{[ji]}\}\Big\}.
\end{align}
We use superscript $R$ and $I$ to denote the real and imaginary parts of the channels ($h_d^{[ji]},h_{m}^{[j]}$ and $g_{m}^{[i]}$) and rewrite \eqref{eq:e_xy_ini} as
\begin{align}
\label{eq:e_xy_first_zeros}
    \mathbb{E}(XY)&=\mathbb{E}\Big\{\Big[\sum_{m=1}^M(g_{m}^{[i]R}h_{m}^{[j]R}-g_{m}^{[i]I}h_{m}^{[j]I})cos \theta_m-(g_{m}^{[i]I}h_{m}^{[j]R}+g_{m}^{[i]R}h_{m}^{[j]I})sin \theta_m+h_d^{[ji]R}\Big] \\ \nonumber &\times \Big[\sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]R}-g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]I})sin \theta_{m^{\prime}}+(g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]R}+g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]I})cos \theta_{m^{\prime}}+h_d^{[ji]I}\Big]\Big\}\\ \nonumber
    &\overset{(b)}{=}\underbrace{\mathbb{E}\{h_d^{[ji]R}h_d^{[ji]I}\}}_{=0}+\underbrace{\mathbb{E}\Big\{\Big[\sum_{m=1}^M(g_{m}^{[i]R}h_{m}^{[j]R}-g_{m}^{[i]I}h_{m}^{[j]I})cos \theta_m-(g_{m}^{[i]I}h_{m}^{[j]R}+g_{m}^{[i]R}h_{m}^{[j]I})sin \theta_m\Big]h_d^{[ji]I}\Big\}}_{=0}\\ \nonumber
    &+\underbrace{\mathbb{E}\Big\{\Big[\sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]R}-g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]I})sin \theta_{m^{\prime}}+(g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]R}+g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]I})cos \theta_{m^{\prime}}\Big]h_d^{[ji]R}\Big\}}_{=0} \\ \nonumber
    &+\mathbb{E}\Big\{\Big[\sum_{m=1}^M(g_{m}^{[i]R}h_{m}^{[j]R}-g_{m}^{[i]I}h_{m}^{[j]I})cos \theta_m-(g_{m}^{[i]I}h_{m}^{[j]R}+g_{m}^{[i]R}h_{m}^{[j]I})sin \theta_m\Big] \\ \nonumber 
    &\times \Big[\sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]R}-g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]I})sin \theta_{m^{\prime}}+(g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]R}+g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]I})cos \theta_{m^{\prime}}\Big]\Big\},
\end{align}
where $(b)$ is correct since $h_d^{[ji]R}$, $h_d^{[ji]I}$, $h_{m}^{[j]R},g_{m}^{[i]R}$, $h_{m}^{[j]I},g_{m}^{[i]I}$,$h_{m^{\prime}}^{[j]R},g_{m^{\prime}}^{[i]R}$, $h_{m^{\prime}}^{[j]I}$, and $g_{m^{\prime}}^{[i]I}$ are independent and $\mathbb{E}\{h_d^{[ji]R}\}=\mathbb{E}\{h_d^{[ji]I}\}=0$. Then, we derive $\mathbb{E}(XY)$ through two cases: (i) $m=m^{\prime}$; (ii) $m\neq m^{\prime}$. Below, we describe these cases.

$\bullet~\mathbf{m=m^{\prime}:}$ In this case, since $m=m^{\prime}$ and $\mathbb{E}(XY)$ should hold for any given value of $M$, we consider $M=1$ and simplify \eqref{eq:e_xy_first_zeros} as
\begin{align}
\label{eq:m_m_complete}
    &\mathbb{E}(XY)\\ \nonumber
    &=\mathbb{E}\Big\{\Big[(g_{m}^{[i]R}h_{m}^{[j]R}-g_{m}^{[i]I}h_{m}^{[j]I})cos \theta_m-(g_{m}^{[i]I}h_{m}^{[j]R}+g_{m}^{[i]R}h_{m}^{[j]I})sin \theta_m\Big] \\ \nonumber 
    &\times \Big[(g_{m}^{[i]R}h_{m}^{[j]R}-g_{m}^{[i]I}h_{m}^{[j]I})sin \theta_{m}+(g_{m}^{[i]I}h_{m}^{[j]R}+g_{m}^{[i]R}h_{m}^{[j]I})cos \theta_{m}\Big]\Big\}\\ \nonumber
    &= \mathbb{E}\Big\{\Big[(g_{m}^{[i]R}h_{m}^{[j]R}-g_{m}^{[i]I}h_{m}^{[j]I})(g_{m}^{[i]I}h_{m}^{[j]R}+g_{m}^{[i]R}h_{m}^{[j]I})(cos^2\theta_m-sin^2\theta_m)\Big] \\ \nonumber 
    &+\frac{1}{2}\mathbb{E}\Big\{\Big[(g_{m}^{[i]R}h_{m}^{[j]R}-g_{m}^{[i]I}h_{m}^{[j]I})^2-(g_{m}^{[i]I}h_{m}^{[j]R}+g_{m}^{[i]R}h_{m}^{[j]I})^2\Big]sin2\theta_m\Big\}\\ \nonumber
    &=\mathbb{E}\Big\{\Big[(h_{m}^{[j]R})^2-(h_{m}^{[j]I})^2\Big]g_{m}^{[i]R}g_{m}^{[i]I}cos2\theta_m+\Big[(g_{m}^{[i]R})^2-(g_{m}^{[i]I})^2\Big]h_{m}^{[j]R}h_{m}^{[j]I}cos2\theta_m\Big\}\\ \nonumber
    &+\frac{1}{2}\mathbb{E}\Big\{\Big[(g_{m}^{[i]R}h_{m}^{[j]R})^2+(g_{m}^{[i]I}h_{m}^{[j]I})^2-(g_{m}^{[i]I}h_{m}^{[j]R})^2-(g_{m}^{[i]R}h_{m}^{[j]I})^2-4g_{m}^{[i]R}g_{m}^{[i]I}h_{m}^{[j]R}h_{m}^{[j]I}\Big]sin2\theta_m\Big\}\\ \nonumber
    &\overset{(c)}{=}\mathbb{E}\Big\{\Big[(h_{m}^{[j]R})^2-(h_{m}^{[j]I})^2\Big]g_{m}^{[i]R}g_{m}^{[i]I}cos2\theta_m\Big\}+\mathbb{E}\Big\{\Big[(g_{m}^{[i]R})^2-(g_{m}^{[i]I})^2\Big]h_{m}^{[j]R}h_{m}^{[j]I}cos2\theta_m\Big\} \\ \nonumber
    &+\frac{1}{2}\Big(\mathbb{E}\Big\{(h_{m}^{[j]R})^2\big[(g_{m}^{[i]R})^2-(g_{m}^{[i]I})^2\big]\Big\}+\mathbb{E}\Big\{(h_{m}^{[j]I})^2\big[(g_{m}^{[i]I})^2-(g_{m}^{[i]R})^2\big]\Big\}\Big)sin2\theta_m \\ \nonumber
    &-2\mathbb{E}\Big\{g_{m}^{[i]R}g_{m}^{[i]I}h_{m}^{[j]R}h_{m}^{[j]I}\Big\}sin2\theta_m\\ \nonumber
    &\overset{(d)}{=}\mathbb{E}\Big\{\Big[(h_{m}^{[j]R})^2-(h_{m}^{[j]I})^2\Big]\Big\}\mathbb{E}\Big\{g_{m}^{[i]R}g_{m}^{[i]I}\Big\}cos2\theta_m+\mathbb{E}\Big\{\Big[(g_{m}^{[i]R})^2-(g_{m}^{[i]I})^2\Big]\Big\}\mathbb{E}\Big\{h_{m}^{[j]R}h_{m}^{[j]I}\Big\}cos2\theta_m \\ \nonumber
    &+\frac{1}{2}\Big(\mathbb{E}\Big\{(h_{m}^{[j]R})^2\Big\}\mathbb{E}\Big\{\big[(g_{m}^{[i]R})^2-(g_{m}^{[i]I})^2\big]\Big\}+\mathbb{E}\Big\{(h_{m}^{[j]I})^2\Big\}\mathbb{E}\Big\{\big[(g_{m}^{[i]I})^2-(g_{m}^{[i]R})^2\big]\Big\}\Big)sin2\theta_m\\ \nonumber
    &-2\mathbb{E}\Big\{h_{m}^{[j]R}h_{m}^{[j]I}\Big\}\mathbb{E}\Big\{g_{m}^{[i]R}g_{m}^{[i]I}\Big\}sin2\theta_m\\ \nonumber
    &\overset{(e)}{=}\underbrace{\mathbb{E}\Big\{\Big[(h_{m}^{[j]R})^2-(h_{m}^{[j]I})^2\Big]\Big\}}_{=0}\mathbb{E}\Big\{g_{m}^{[i]R}g_{m}^{[i]I}\Big\}cos2\theta_m+\underbrace{\mathbb{E}\Big\{\Big[(g_{m}^{[i]R})^2-(g_{m}^{[i]I})^2\Big]\Big\}}_{=0}\mathbb{E}\Big\{h_{m}^{[j]R}h_{m}^{[j]I}\Big\}cos2\theta_m \\ \nonumber
    &+\frac{1}{2}\Big(\mathbb{E}\Big\{(h_{m}^{[j]R})^2\Big\}\underbrace{\mathbb{E}\Big\{\big[(g_{m}^{[i]R})^2-(g_{m}^{[i]I})^2\big]\Big\}}_{=0}+\mathbb{E}\Big\{(h_{m}^{[j]I})^2\Big\}\underbrace{\mathbb{E}\Big\{\big[(g_{m}^{[i]I})^2-(g_{m}^{[i]R})^2\big]\Big\}}_{=0}\Big)sin2\theta_m \\ \nonumber
    &-2\mathbb{E}\Big\{h_{m}^{[j]R}h_{m}^{[j]I}\Big\}\underbrace{\mathbb{E}\Big\{g_{m}^{[i]R}g_{m}^{[i]I}\Big\}}_{=0}\Big)sin2\theta_m=0,
\end{align}
where $(c)$ happens since the expected value operator is linear, and $(d)$ and $(e)$ are true because (i) the real and imaginary parts of the channels are independent; (ii) $\mathbb{E}\Big\{(g_{m}^{[i]I})^2\Big\}=\mathbb{E}\Big\{(g_{m}^{[i]R})^2\Big\}$; (iii) $\mathbb{E}\Big\{g_{m}^{[i]R}\Big\}=\mathbb{E}\Big\{g_{m}^{[i]I}\Big\}=0$.

$\bullet~\mathbf{m\neq m^{\prime}}:$ In this case, we have
\begin{align}
\label{eq:four_terms}
    \mathbb{E}(XY)&=\mathbb{E}\Big\{\Big[\sum_{m=1}^M(g_{m}^{[i]R}h_{m}^{[j]R}-g_{m}^{[i]I}h_{m}^{[j]I})cos \theta_m-(g_{m}^{[i]I}h_{m}^{[j]R}+g_{m}^{[i]R}h_{m}^{[j]I})sin \theta_m\Big] \\ \nonumber 
    &\times \Big[\sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]R}-g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]I})sin \theta_{m^{\prime}}+(g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]R}+g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]I})cos \theta_{m^{\prime}}\Big]\Big\}.
\end{align}

Then, we use the linear property of the expected value operator and break \eqref{eq:four_terms} into four terms as \eqref{eq:first_product}, \eqref{eq:second_product}, \eqref{eq:third_product}, and \eqref{eq:fourth_product}. Here are the details.
\begin{align}
\label{eq:first_product}
    &\mathbb{E}\Big\{\sum_{m=1}^M(g_{m}^{[i]R}h_{m}^{[j]R}-g_{m}^{[i]I}h_{m}^{[j]I})cos \theta_m\times \sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]R}-g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]I})sin \theta_{m^{\prime}}\Big\} \\ \nonumber
    &\overset{(f)}{=}\mathbb{E}\Big\{\sum_{m=1}^M(g_{m}^{[i]R}h_{m}^{[j]R})cos \theta_m \sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]R})sin \theta_{m^{\prime}}\Big\}-\mathbb{E}\Big\{\sum_{m=1}^M(g_{m}^{[i]I}h_{m}^{[j]I})cos \theta_m \sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]R})sin \theta_{m^{\prime}}\Big\} \\ \nonumber
    &+\mathbb{E}\Big\{\sum_{m=1}^M(g_{m}^{[i]I}h_{m}^{[j]I})cos \theta_m \sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]I})sin \theta_{m^{\prime}}\Big\}-\mathbb{E}\Big\{\sum_{m=1}^M(g_{m}^{[i]R}h_{m}^{[j]R})cos \theta_m \sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]I})sin \theta_{m^{\prime}}\Big\} \\ \nonumber
    &\overset{(g)}{=}\mathbb{E}\Big\{\sum_{m=1}^M(g_{m}^{[i]R}h_{m}^{[j]R})cos \theta_m\Big\} \mathbb{E}\Big\{\sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]R})sin \theta_{m^{\prime}}\Big\} \\ \nonumber
    &-\mathbb{E}\Big\{\sum_{m=1}^M(g_{m}^{[i]I}h_{m}^{[j]I})cos \theta_m\Big\} \mathbb{E}\Big\{\sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]R})sin \theta_{m^{\prime}}\Big\} \\ \nonumber
    &+\mathbb{E}\Big\{\sum_{m=1}^M(g_{m}^{[i]I}h_{m}^{[j]I})cos \theta_m\Big\} \mathbb{E}\Big\{\sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]I})sin \theta_{m^{\prime}}\Big\} \\ \nonumber
    &-\mathbb{E}\Big\{\sum_{m=1}^M(g_{m}^{[i]R}h_{m}^{[j]R})cos \theta_m \Big\}\mathbb{E}\Big\{\sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]I})sin \theta_{m^{\prime}}\Big\}\\ \nonumber
    &\overset{(h)}{=}\sum_{m=1}^M\underbrace{\mathbb{E}\{g_{m}^{[i]R}\}}_{=0}\mathbb{E}\{h_{m}^{[j]R}cos \theta_m\} \sum_{m^{\prime}=1}^M\underbrace{\mathbb{E}\{g_{m^{\prime}}^{[i]R}\}}_{=0}\mathbb{E}\{h_{m^{\prime}}^{[j]R}sin \theta_{m^{\prime}}\}\\ \nonumber
    &-\sum_{m=1}^M\underbrace{\mathbb{E}\{g_{m}^{[i]I}\}}_{=0}\mathbb{E}\{h_{m}^{[j]I}cos \theta_m\} \sum_{m^{\prime}=1}^M\underbrace{\mathbb{E}\{g_{m^{\prime}}^{[i]R}\}}_{=0}\mathbb{E}\{h_{m^{\prime}}^{[j]R}sin \theta_{m^{\prime}}\} \\ \nonumber
    &+\sum_{m=1}^M\underbrace{\mathbb{E}\{g_{m}^{[i]I}\}}_{=0}\mathbb{E}\{h_{m}^{[j]I}cos \theta_m\} \sum_{m^{\prime}=1}^M\underbrace{\mathbb{E}\{g_{m^{\prime}}^{[i]I}\}}_{=0}\mathbb{E}\{h_{m^{\prime}}^{[j]I}sin \theta_{m^{\prime}}\}\\ \nonumber
    &-\sum_{m=1}^M\underbrace{\mathbb{E}\{g_{m}^{[i]R}\}}_{=0}\mathbb{E}\{h_{m}^{[j]R}cos \theta_m \}\sum_{m^{\prime}=1}^M\underbrace{\mathbb{E}\{g_{m^{\prime}}^{[i]I}\}}_{=0}\mathbb{E}\{h_{m^{\prime}}^{[j]I}sin \theta_{m^{\prime}}\}=0,
\end{align}
where $(f)$ follows the linear property of the expected value operator, and $(g)$ and $(h)$ are true because $h_d^{[ji]R}$, $h_d^{[ji]I}$, $h_{m}^{[j]R},g_{m}^{[i]R}$, $h_{m}^{[j]I},g_{m}^{[i]I}$,$h_{m^{\prime}}^{[j]R},g_{m^{\prime}}^{[i]R}$, $h_{m^{\prime}}^{[j]I}$, and $g_{m^{\prime}}^{[i]I}$ are independent.
Similar to \eqref{eq:first_product}, we can show that
\begin{align}
\label{eq:second_product}
    \mathbb{E}\Big\{\sum_{m=1}^M(g_{m}^{[i]R}h_{m}^{[j]R}-g_{m}^{[i]I}h_{m}^{[j]I})cos \theta_m\times \sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]R}-g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]I})cos \theta_{m^{\prime}}\Big\}=0,
\end{align}
\begin{align}
\label{eq:third_product}
    \mathbb{E}\Big\{\sum_{m=1}^M(g_{m}^{[i]I}h_{m}^{[j]R}-g_{m}^{[i]R}h_{m}^{[j]I})sin \theta_m\times \sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]R}-g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]I})sin \theta_{m^{\prime}}\Big\}=0,
\end{align}

\begin{align}
\label{eq:fourth_product}
    \mathbb{E}\Big\{\sum_{m=1}^M(g_{m}^{[i]I}h_{m}^{[j]R}-g_{m}^{[i]R}h_{m}^{[j]I})sin \theta_m\times \sum_{m^{\prime}=1}^M(g_{m^{\prime}}^{[i]I}h_{m^{\prime}}^{[j]R}-g_{m^{\prime}}^{[i]R}h_{m^{\prime}}^{[j]I})sin \theta_{m^{\prime}}\Big\}=0.
\end{align}

Therefore, using \eqref{eq:m_m_complete}, \eqref{eq:first_product}, \eqref{eq:second_product}, \eqref{eq:third_product}, and \eqref{eq:fourth_product} prove that $\mathbb{E}\{XY\}=0$, and this means that $X$ and $Y$ are independent.

As a result, for $j\in\{1,2,\ldots,K\}, j\neq i.$ we simplify \eqref{eq:intersect_real_imag} as 
\begin{align}
    &\Pr\Big(\Big|\textbf{g}^{[i]}\mathbf{\Theta}\textbf{h}^{[j]}+h_d^{[ji]}\Big|<\delta\Big|\mathbf{\Theta}\Big) \\ \nonumber
    &>\Pr\Big(\Big|Re\{\textbf{g}^{[i]}\mathbf{\Theta}\textbf{h}^{[j]}+h_d^{[ji]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta}\Big)\Pr\Big(\Big|Im\{\textbf{g}^{[i]}\mathbf{\Theta}\textbf{h}^{[j]}+h_d^{[ji]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta}\Big).
\end{align}
Since $Re\{\textbf{g}^{[i]}\mathbf{\Theta}\textbf{h}^{[j]}+h_d^{[ji]}\}$ is a zero-mean Gaussian random variable, we have
\begin{align}
    \Pr\Big(\Big|Re\{\textbf{g}^{[i]}\mathbf{\Theta}\textbf{h}^{[j]}+h_d^{[ji]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta}\Big)&=\int_{-\frac{\delta}{\sqrt{2}}}^{\frac{\delta}{\sqrt{2}}}\frac{1}{\sqrt{\pi \nu}}e^{\frac{-r^2}{\nu}}dr \\ \nonumber
    &\overset{(q)}{\approx}\int_{-\frac{\delta}{\sqrt{2}}}^{\frac{\delta}{\sqrt{2}}}\frac{1}{\sqrt{\pi \nu}}\Big[1-\frac{r^2}{\nu}+O (\frac{r^4}{\nu^2})\Big]dr\\ \nonumber
    &=\frac{1}{\sqrt{\pi \nu}} \Big[\sqrt{2}\delta-\frac{\delta^3}{3\sqrt{2}\nu}+O(\frac{r^5}{\nu^2}) \Big]\\ \nonumber
    &\overset{(\ell)}{\approx}(\frac{\sqrt{2}\delta}{\sqrt{\pi \nu}}), ~~ j\in\{1,2,\ldots,K\}, j\neq i,
\end{align}
where $(q)$ applies based on approximation from the Taylor expansion of $e^{\frac{-r^2}{\nu}}$, and $(\ell)$ holds since our goal is to have small $\delta$; therefore, we ignore the high orders of $\frac{r}{\nu}$.

Similarly, we obtain
\begin{align}
    \Pr\Big(\Big|Im\{\textbf{g}^{[i]}\mathbf{\Theta}\textbf{h}^{[j]}+h_d^{[ji]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta}\Big)\approx(\frac{\sqrt{2}\delta}{\sqrt{\pi \nu}}), ~~ j\in\{1,2,\ldots,K\}, j\neq i.
\end{align}

Hence, using (24) and (25) leads to
\begin{align}
    \Pr\Big(\Big|\textbf{g}^{[i]}\mathbf{\Theta}\textbf{h}^{[j]}+h_d^{[ji]}\Big|<\delta\Big|\mathbf{\Theta}\Big)&>(\frac{\sqrt{2}\delta}{\sqrt{\pi \nu}})^2, j\in\{1,2,\ldots,K\}, j\neq i,
\end{align}
which completes the proof.
\end{proof}

==> sections/Introduction.tex <==
A massive ecosystem of connected devices is predicted to reach about 100 billion devices by 2025~\cite{mc_global_link}, and the Internet of Things (IoT) network, as a part of this connected ecosystem, is expected to develop at a compound annual growth rate of 20 percent~\cite{IoT_link}. IoT networks enable various applications, such as smart manufacturing, emergency detection, and structural health monitoring~\cite{mozaffari2017mobile}. IoT devices, on the other hand, generally have limited resources due to their small size and hence low battery capacity. Moreover, due to the paucity of spectrum for wireless electromagnetic transmission, base-stations (BSs) and IoT devices are near each other or even overlapping in the spectrum, resulting in co-channel interference.

To handle interference, most architectures rely on massive multiple-input multiple-output
(MIMO) designs, which exploit digital beamforming with full digital precision to cancel out interference in digital domain. However, these methods are power-hungry, with a high implementation cost due to using multiple radio frequency (RF) chains and analog-to-digital converters (ADCs)~\cite{zhang2016fundamental,ngo2013energy}.

\begin{comment}

To handle interference, traditionally, past works utilize massive multiple-input multiple-output
(MIMO) and millimeter wave (mmWave) communications, which exploit digital and phased array beamforming, respectively, to create a beam toward the desired user. However, these methods are power-hungry, with a high implementation cost~\cite{zhang2016fundamental,ngo2013energy,wu2017overview}.
\end{comment}

%The fifth-generation (5G) of wireless networks and beyond are deemed promising technologies for supporting many mobile users with high data rates%{\color{blue}%, which increases the deployment density of base-stations (BSs). Sending signals from BSs toward the users in the same communication channel results in co-channel interference; thus, interference ought to be handled in these networks. 
%To do so, there are some
%existing methods such as massive multiple-input-multiple-output (MIMO) and millimeter wave (mmWave) communications, %{\color{red}Thuan: We should clearly mention how MIMO, mmWave deal with interference. Also, we have many kinds of interference (co-channel interference, noise, thermal,...). It needs to tell specific interference you want to focus on} {\color{blue}
%which exploit digital and phased array beamforming, respectively, to create a beam toward the desired user. However, these methods pose problems for green communications in terms of high power consumption and implementation cost~\cite{zhang2016fundamental,ngo2013energy,wu2017overview}.


\begin{comment}


Using relays is another well-known method to overcome interference. Relays convert
a single non-line-of-sight (NLoS) link into multiple line-of-sight (LoS) links dedicating power source and re-transmission, which increase power consumption. However, relays perform transmission through half-duplex and full-duplex relaying protocols where the former is not a spectral-efficient way due to being silent for half of the time, and the latter suffers from high loop-back
self-interference at the relay, generating co-channel
interference at the destination, and increasing the signal processing complexity and the power
consumption of the relays~\cite{lu2015stochastic}.
\end{comment}

To address the above issues, reconfigurable-intelligent-surface (RIS) has been recently proposed as a promising technology to provide high spectrum efficiency in a low-cost and power-efficient manner. Specifically, an RIS includes $M$ programmable passive reflectors (i.e., phase-shifters (PSs)) to reflect and steer the incident signals toward the desired directions.%. In particular, an RIS includes $M$ passive elements (i.e., phase-shifters (PSs)) and is used to reflect the incident signal through smartly tuning those passive PSs. %Interestingly, RIS is potentially able to improve the strength of the desired signal in $\mathcal{O}(M^2)$, while active relays provide $\mathcal{O}(M)$ signal enhancement~\cite{wu2019intelligent}. %Notice that the RIS-assisted network suffers from a significant path loss from the reflected paths, necessitating the use of large enough RIS elements to compensate for this resultant path loss~\cite{di2020reconfigurable}. 

%{\color{blue}
%{\color{red} you need to mentioned ``Degrees of freedom of two-hop wireless networks: Everyone gets the entire cake''}

Control and placement of intelligent surfaces are two main challenges in 
the RIS-assisted networks. The past works mainly investigated 
the RIS-assisted networks in two categories. First,~\cite{bafghi2022degrees,gan2021user} focused on single-input single-output (SISO) networks and studied degrees-of-freedom (DoF) and ergodic rate to evaluate performance. In particular,~\cite{bafghi2022degrees} showed that DoF of $K$ (maximum possible value of DoF) could be achieved using either an active RIS with more than $K(K-1)$ elements or a passive RIS with large enough elements. Moreover,~\cite{gan2021user} obtained the ergodic rate for a broadcast channel through user selection and deriving the distribution of the received signal.{\color{red} do not start a sentence with a citation}~\cite{gan2021user} assumed Rician fading for the channels connected to the RIS and obtained that the received signal at receiver and its amplitude are distributed based on Gaussian and Exponential distributions, respectively. However, these solutions did not propose {\color{red} (1) are you sure? (2)how many the tens opf papers that do optimize the RIS??} how to control the RIS elements. In this paper, we optimize the RIS elements to maximize sum-rate and study the max-min optimization problem to meet fairness between users. {\color{red} how is this last sentence related to control?!} We also derive a lower-bound on the minimum number of RIS elements to meet a certain performance.

\begin{comment}
Researchers have investigated several interference suppression techniques in RIS-assisted networks from both theoretical and practical standpoints~\cite{bafghi2022degrees,fu2021reconfigurable,kammoun2020asymptotic,yu2020power,zhi2021two}. Theoretically, obtaining the precise capacity expressions for multi-user communication channels is challenging. As a result, the literature typically defines the degrees-of-freedom %{\color{red} it is degrees not degree, please apply everywhere} 
(DoF) as a more tractable metric for characterizing the performance of interference suppression methods, where DoF is the pre-log factor in the sum-rate equation. DoF is often computed in interference channels, which are motivated by cellular networks especially with cell-edge users. More precisely, in a $K$-user interference channel, each transmitter wishes to communicate with one desired user while other interfering transmitters are present. It has been demonstrated in~\cite{cadambe2008interference} that the DoF of $K/2$ is achievable without the use of RIS. It is worth noting that the eventual value of the DoF can be equal to $K$ if each transmitter delivers its messages to its desired receiver without interference. In~\cite{shomorony2014degrees}, the authors showed that the DoF of $K$ is achievable by exploiting $K$ relays under time-varying and constant channel coefficients. Further, in~\cite{vahid2015informational,vahid2019degrees}, the impact of imperfect CSI on two-unicast networks with relays was studied. However, the relay-aided networks are power hungry and increase complexity. On the other hand, recently~\cite{bafghi2022degrees} studied the DoF of a time-selective $K$-user interference channel in the presence of an RIS. It showed that an active RIS (i.e., each RIS element incorporates both amplifier and reflector) with more than $K(K-1)$ elements can achieve a DoF of $K$. Furthermore,~\cite{bafghi2022degrees} presented a probabilistic lower bound for the DoF with a passive RIS, which approaches $K$ as the number of RIS elements tends to infinity. Authors in~\cite{fu2021reconfigurable} analyzed the DoF in a MIMO context with rank-deficient channels and applied the RIS and beamforming at the transmitters and receivers to enhance the DoF over a no-RIS scenario. However, these solutions need the availability of global channel-state-information (CSI) at the BSs, which is a bottleneck in practice due to the necessity for excessive overhead, especially when taking into account the large number of channels in the presence of the RIS. Additionally, these results focus on high signal-to-noise-ratio (SNR) regimes (i.e., SNR$\to \infty$) to study DoF, which is not feasible in practice.
\end{comment}


{\color{red} no idea what your two categories are! How are these works separated? This part is very poorly written. Are you talking about control and placement or information theory vs. networking?} Second, other literature considered beamforming techniques to control the RIS and thus handle interference. Specifically,~\cite{kammoun2020asymptotic,yu2020power,zhi2021two} used a single RIS (referred to as a centralized RIS) in a broadcast channel and managed interference through optimizing the beamformer at the transmitter and the RIS elements. In these works, the single RIS
is located usually close to either transmitter or receivers due to the intensive product path loss between BSs and users through the RIS. 

On the other hand, single-RIS-assisted networks face some limitations: (1) the single-RIS coverage area is limited as it only serves users in the reflection half-space, and (2) it is not always possible to establish a blockage-free link between the BS and users through the RIS (e.g., multi-turn corridors), and (3) due to practical constraints on the physical size of each RIS element, the single RIS may only offer limited passive beamforming gain and hence cannot assist boosting the sum-rate significantly. As a result,~\cite{zheng2021uplink,li2021double} proposed a cooperated passive beamforming using two RISs, with one RIS located near the BS and the other near a cluster of users; however, placing one RIS nearby the mobile users is not a realistic assumption.

In addition to control and placement of the RIS elements, the aforementioned methods considered two impractical assumptions: (1) They assumed that each PS has infinite bit resolution, which makes the implementation hard~\cite{huang2017dynamical}. 
%In addition, it is unknown whether the gain of $\mathcal{O}(M^2)$ is achievable with low-bit PSs since it is not possible to align the interference signals perfectly~\cite{wu2019intelligent}. 
Then,~\cite{wu2019beamforming,abdullah2022low} exploited low-bit PSs and proposed optimization methods based on successive-refinement (SR), which optimizes each RIS element individually; (2) They offered solutions based on the availability of accurate channel state information (CSI) at all nodes, including transmitters. We refer to this as ``global perfect CSI.'' However, assuming global perfect CSI is practically impossible due to channel estimation errors during the training phase before communication and the need for significant feedback for CSI to be available at all nodes.
%-------
%Motivated by the above, we study a downlink single-input single-output (SISO) IoT network in this paper. We assume two RIS cases: (1) a centralized RIS and (2) $K$ distributed RISs with one dedicated RIS to each transmitter, which can be implemented in a real-world industrial IoT network, where each RIS is installed on the factory facade close to its associated transmitter. We assume that global CSI is available at all nodes in the first case, while each transmitter knows only its outgoing channel to the receivers (referred to as local channel state information at transmitter or local CSIT), and beyond that, it is only aware of the statistics of other channels in the second case. We consider low-bit PSs at the RIS(s) and optimize the RIS elements to maximize sum-rate. Moreover, we study the max-min optimization problem to meet fairness between users. %In this work, we use filled function optimization method to optimize the objective functions. 
%Here are the main contributions of this paper:



Motivated by the above, we exploit low-bit PSs at RIS and optimize the RIS elements. Moreover, we consider imperfect CSI, where the channels are estimated with errors, and then assume two RIS cases: (1) a centralized RIS and (2) $K$ distributed RISs with one dedicated RIS to each transmitter. We assume that global CSI is available at all nodes in the first case, while each transmitter knows only its outgoing channel to the receivers (referred to as local channel state information at the transmitter or local CSIT), and beyond that, it is only aware of the statistics of other channels in the second case. To locate the RISs, in a centralized RIS, we shift the RIS between the transmitter and
receiver and obtain the minimum number
of RIS elements to meet a specific performance at different positions. Then, in the distributed case, we assign one RIS to each transmitter and place each RIS close to its dedicated transmitter. %We consider low-bit PSs at the RIS(s) and optimize the RIS elements to maximize sum-rate. Moreover, we study the max-min optimization problem to meet fairness between users. %In this work, we use filled function optimization method to optimize the objective functions. 
Here are the main contributions of this paper:

\begin{itemize}
    \item We present a low-cost and power-efficient solution to suppress interference in a SISO network by leveraging centralized and distributed RISs. The former strategy needs global imperfect CSI at the transmitters, and the latter uses local imperfect CSIT to optimize the RIS elements. We show numerically that the distributed RISs have a higher sum-rate than a centralized RIS and require fewer components to achieve a specific performance;
    \item %{\color{blue}
    We show via simulation that our proposed solution via distributed RISs provides the DoF of $K$ in low-to-moderate SNR values, and we provide outage capacity analysis;
    \item We assume a low-bit phase shifter at each RIS element, resulting in a nonlinear integer programming (NLIP) problem. We propose an optimization method based on a sigmoid filled function to optimize the PSs. We compare our approach to a simplified exhaustive search (SES) method, the genetic algorithm (GA), and two SR-based methods~\cite{wu2019beamforming,abdullah2022low}
    in terms of sum-rate and complexity. We observe that our method outperforms the benchmarks with a reasonable complexity; %when the channels are estimated in the presence of a random noise before communication;
    \item We derive a lower bound on the minimum number of RIS elements required to attain a certain performance.
\end{itemize}

The rest of the paper is structured as follows. We present our channel model based on centralized and distributed RISs, and outline the optimization problem in Section~\ref{Section:Problem}. In Section~\ref{Section:opt_approach}, we discuss our proposed optimization approach. Then, in Section~\ref{Section:min_M}, we provide a lower bound on the minimum number of RIS elements. In Section~\ref{Section:Numerical}, we present the simulation results and then conclude the paper in Section~\ref{Section:conclusion}.
\subsection{Notations}
Throughout the paper, we use bold-face lowercase, bold-face uppercase, and italic letters to denote vectors, matrices, and scalars, respectively. We also use $\mathbb{C}^{I\times J}$ to describe the space of $I\times J$ complex-valued matrices. $\mathrm{diag}\{\textbf{x}\}$ is a diagonal matrix using vector $\textbf{x}$, and $|\textbf{x}|$ and $||\textbf{x}||$ are the absolute value and Euclidean norm of complex-valued vector $\textbf{x}$, respectively. % In this work, $\textbf{I}_K$ represents the identity matrix with size $K\times K$. 
We use $\mathbb{E}(.)$, $\log(.)$, $Re(.)$, and $Im(.)$ to denote the statistical expectation, logarithmic function in base 2, and real and imaginary parts of a complex number, respectively. Finally, $\textbf{B}^H$ shows the conjugate transpose of matrix $\textbf{B}$.

==> sections/Section3_main_results.tex <==
%As we mentioned earlier, the optimization method based on filled function works with any nonlinear objective function as long as the only constraint is to select choices from a discrete domain. 
This section represents the main results of our interference suppression methods using a centralized RIS and $K$ distributed RISs. To demonstrate the results, we first explain our optimization methods based on filled function and then show a lower bound on the minimum number of elements at RIS(s) to achieve a specific performance. Further details are described below:
\subsection{Centralized RIS}
% To simplify the descriptions of our optimization method, we use a dual format of \eqref{eq:opt_max} as {\color{red} introduce $q$ in (10), waste of space for something trivial} 
% \begin{align}
% \label{eq:opt_min_one_RIS}
%     &\underset{\boldsymbol{\theta}}{\min}~q(\boldsymbol{\theta})=-\sum_{i=1}^{K} \log(1+\text{SINR}_i)\\ \nonumber
%     &\text{s.t.} ~~ \boldsymbol{\theta}=[\theta_1,\theta_2,\ldots,\theta_{M}], ~~ \theta_{m}\in \phi_N \quad~ \text{for}~ 1\leq m \leq M.
% \end{align}

% In this case, since there is only one RIS to assist the users, we omit superscript $i$ from the descriptions of RIS. We substitute $q(\mathbf{\Theta})$ with $q(\boldsymbol{\theta})$ where $q(\boldsymbol{\theta})=q(diag\{e^{j\boldsymbol{\theta}}\})$ and revise the optimization problem in \eqref{eq:opt_min} as 
% \begin{align}
% \label{eq:opt_min_one_RIS}
%     &\underset{\boldsymbol{\theta}}{\min}~ q(\boldsymbol{\theta})\\ \nonumber
%     &\text{s.t.} ~~ \boldsymbol{\theta}=[\theta_1,\theta_2,\ldots,\theta_{M}], ~~ \theta_{m}\in \phi_N \quad~ \text{for}~ 1\leq m \leq M.
% \end{align}

\subsubsection{Optimization method}
\label{sub_subsect_optim_central_RIS}

The idea of utilizing an optimization approach based on a filled function was originally introduced in~\cite{renpu1990filled} for the continuous domain. Then,~\cite{ng2005discrete} updated it for the discrete domain. In this paper, we use a sigmoid-based filled function %~\cite{binary_switch_sajjad}
and run local and global searches to optimize \eqref{eq:opt_min_one_RIS}.

%-----------
\textbf{Local search:}
We define $\mathcal{N}(\boldsymbol{\theta})$ as the neighbors of an RIS configuration $\boldsymbol{\theta}$ such that
\begin{align}
    \mathcal{N}(\boldsymbol{\theta})=\boldsymbol{\theta} \cup \{\boldsymbol{\theta}+\mathbf{\bm{\lambda}}_m,\mathbf{\bm{\lambda}}_m\in \bm{\Lambda}\}
\end{align}
where $\mathbf{\bm{\lambda}}_m$ is an $M$-length column vector with the $\text{m}^\text{th}$ element chosen from $\{0,\frac{2\pi}{N},\frac{4\pi}{N},\ldots,$ $\frac{2\pi(N-1)}{N}\}$ and the others equal to zero; further $\bm{\Lambda}$ is the direction set equals to $\bm{\Lambda}=\{\mathbf{\bm{\lambda}}_m, m=1,2,\ldots, M\}$. Here, the local search scans all neighbors of $\boldsymbol{\theta}$ to find a solution as $\boldsymbol{\theta}^* \in \mathcal{N}(\boldsymbol{\theta})$ such that $q(\boldsymbol{\theta}^*) \leq q(\boldsymbol{\theta})$. If $\boldsymbol{\theta}^*=\boldsymbol{\theta}$, we call $\boldsymbol{\theta}^*$ the local minimizer; otherwise, we consider $\boldsymbol{\theta}=\boldsymbol{\theta}^*$ and repeat the local search.

\textbf{Global search:} The filled function plays an important role in the global search. In this work, we use sigmoid-based filled function $Q_r(\boldsymbol{\theta},\boldsymbol{\theta}^*)$ and define an auxiliary optimization problem as
\begin{comment}
In~\cite{renpu1990filled}, the authors provide three necessary conditions that any filled function must meet. To satisfy these conditions,~\cite{zhu1998approximate,ng2005discrete} exploit two heuristic parameters, which causes some difficulties in modifying these parameters to match the conditions. Then,~\cite{gu2006new,binary_switch_sajjad} propose the filled functions with a single parameter and \cite{binary_switch_sajjad} mentions that its sigmoid filled function is faster than some known filled function. Therefore, in this work, we use the sigmoid filled function as $Q_r(\boldsymbol{\theta},\boldsymbol{\theta}^*)$ where $\boldsymbol{\theta}^*$ is the current local minimizer of \eqref{eq:opt_min_one_RIS} and $r>0$ describes the filled function parameter. We interpret $r$ as a radius around $\boldsymbol{\theta}^*$ that we would like to search for the global solution. Of course, increasing $r$ enhances the results, but increases the complexity.
\end{comment}
\begin{align}
\label{eq:aux_opt}
    \underset{\boldsymbol{\theta}}{\min}~Q_r(\boldsymbol{\theta},\boldsymbol{\theta}^*)\\ \nonumber
    \text{s.t.} \quad \boldsymbol{\theta},\boldsymbol{\theta}^*\in \phi_N,
\end{align}
where $\boldsymbol{\theta}^*$ is the current local minimizer of \eqref{eq:opt_min_one_RIS} and $r>0$ denotes the filled function parameter. The aim here is to find a better solution than $\boldsymbol{\theta}^*$. To do so, we apply $\boldsymbol{\theta}^*$ to the filled function and run the local search for \eqref{eq:aux_opt} to get $\bar{\boldsymbol{\theta}^*}$. Finally, we use $\bar{\boldsymbol{\theta}^*}$ as the input of the local search with \eqref{eq:opt_min_one_RIS} to obtain $\boldsymbol{\theta}^{**}$. If $q(\boldsymbol{\theta}^{**})<q(\boldsymbol{\theta}^*)$, we call $\boldsymbol{\theta}^{**}$ a new solution that outperforms $\boldsymbol{\theta}^*$. Furthermore, in this work, we propose a new strategy to connect \eqref{eq:opt_min_one_RIS} and \eqref{eq:aux_opt} that decreases complexity while resulting in negligible performance loss. We will provide two algorithms in Section~\ref{Section:opt_approach} to demonstrate the details of how our optimization method performs.

To meet fairness among users, we define a max-min optimization problem as
\begin{align}
\label{eq:opt_min_one_RIS_fairness}
    &\underset{\boldsymbol{\theta}}{\max}\underset{i=\{1,2,\ldots,K\}}{\min} \log(1+\text{SINR}_i)\\ \nonumber
    &\text{s.t.} ~~ \boldsymbol{\theta}=[\theta_1,\theta_2,\ldots,\theta_{M}], ~~ \theta_{m}\in \phi_N \quad~ \text{for}~ 1\leq m \leq M.
\end{align}
%{\color{red} this should be a remark} 
\begin{remark}
We note that the filled function-based optimization methods can optimize a general nonlinear objective function as long as selecting a possible configuration from a discrete set is the only constraint. This model is usually referred to as unconstrained optimization problem~\cite{ng2005discrete}.
\end{remark}%}{\color{red} the next sentence is not needed.} %As a result, we use the same optimization approach based on sigmoid filled function to find the optimal solution in \eqref{eq:opt_min_one_RIS_fairness}.
%-----------


\subsubsection{Lower bound on the minimum number of RIS elements}
\label{sub_subsect_lower_bound_central_RIS}

We provide a lower bound on the minimum number of RIS elements to ensure that each receiver gets a specific value of SINR denoted by $\Tilde{\text{SINR}}$. To do this, we consider a symmetric scenario, which includes the following: (i) All transmitters have the same transmit power (i.e., $P_i=P, i \in \{1,2,,\ldots K\}$); Each receiver stands at the same distance from all transmitters; (iii) The distance between the RIS and all transmitters are the same; (iv) The receivers are placed at the same distance from the RIS. %{\color{blue} 
The main idea here is to assume that the RIS elements are independent of the channel coefficients and then utilize that assumption to obtain an asymptotic distribution for $\textbf{g}^{[i]}\mathbf{\Theta}\textbf{h}^{[j]}+h_d^{[ji]}, i,j=1,2,\dots,K$. Finally, we derive the lower bound on $M$ for a practical interval, $10<M<512$ %{\color{red} strict inequality?} 
as
 \begin{align}
 \label{eq:lower_bound_main_results}
    M>\underset{a}{\min}\Big\{K(K-1)\log_N\Big[\frac{\Tilde{\text{SINR}}\frac{\pi}{2}(K-1)(\sigma_{h_d}^2+512\nu^{\prime})}{(\sigma_{h_d}^2+10\nu^{\prime})\Big[Q^{-1}\big(\frac{1}{2N^{a/2}}\big)\Big]^2-\frac{\Tilde{\text{SINR}}\sigma^2}{P}}\Big]+a\Big\},
\end{align}
%{\color{red}Thuan: How can we obtain this eq.? or we should add relevant reference. }
where $Q^{-1}(.)$ is the inverse of Q-function, $\log_N$ is a logarithmic function in base $N$,
\begin{align}
    \nu^{\prime}=(m_h)^2\sigma_g^2,
\end{align}
and $a$ shows a trade-off between signal enhancement from the desired transmitter and suppressing the interference signals from other transmitters. For instance, we use $a=0$ to dedicate RIS elements to reduce the interference and $a=M$ to exploit RIS elements to improve the desired signal. We will provide a detailed description in Section~\ref{Section:min_M}. 

We define $M_{\min}$ as the smallest integer that satisfies \eqref{eq:lower_bound_main_results}. Furthermore, we refer to the curve that shows the average SINR versus different values of $P$ using $M_{\min}$ RIS elements as the theoretical-bound. In Section~\ref{Section:Numerical}, we will demonstrate a comparison result between our optimization method and the theoretical-bound. 
\subsection{Distributed RISs}
\label{subsect:main_result_dist_RIS}
In this case, we define $score_i$ as a new objective function that captures the fact of enhancing the desired signals from ${\sf Tx}_i, i=1,2,\ldots,K$ at ${\sf Rx}_i$ while suppressing the interference signals from ${\sf Tx}_i$ at other receivers. Consequently, we write $score_i$ as
\begin{align}
\label{eq:score_i}
    score_i \triangleq\frac{P_i\Big|\textbf{g}^{[ii]}\mathbf{\Theta}^{[i]}\textbf{h}^{[ii]}+h_d^{[ii]}\Big|^2}{\sigma^2+\sum_{j=1, j\neq i}^{K}P_i\Big|\textbf{g}^{[ij]}\mathbf{\Theta}^{[i]}\textbf{h}^{[ii]}+h_d^{[ij]}\Big|^2},
\end{align}
%{\color{blue}
where compared to $\text{SINR}_i$ given in \eqref{eq:SINR_update_a_RIS}, the denominator includes noise and the interference caused by ${\sf Tx}_i$ at unintended receivers.
%{\color{red}Say something like the following but make sure it is accurate: compared to SINR given in (6), the denominator is the interference caused by $Tx_i$ at unintended receivers}
\begin{figure}[ht]
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.99\linewidth, draft=false]{images/sinr_sir_snr_3.png}
  \caption{\it %{\color{red}Thuan: in legend, we must write exactly $Tx_i$ as in Fig. 1. }
  Sum-rate versus $\log(M)$ with different objective functions as $\text{SNR}_i$, SIR-${\sf Tx}_i$, and $score_i$.%: (1) maximizing the desired signal from ${\sf Tx}_i$ at ${\sf Rx}_i$; (2) maximizing the ratio of the desired signal from ${\sf Tx}_i$ at ${\sf Rx}_i$ over the interference signals from ${\sf Tx}_i$ at undesired receivers; (3) $\max\{score_i\}$. 
  We assume %{\color{red}Thuan: Here, we have 3 RISs, it seems like you mentioned 3 pairs of transmitter-receiver, right? So, sum-rate here is sum of 3 rates of 3 receivers, right?} {\color{blue}
  $K=4$, $N=4$, $\sigma^2=-80$dBm, and $P_i \in \{20, 30, 40\}$ in dBm scale.} 
  \label{Fig:sinr_sir_snr}
\end{figure}
\subsubsection{Optimization method}
\label{sub_subsect_optim_dist_RIS}
We define the optimization problem based on $score_i$ as follows:
\begin{align}
\label{eq:opt_max_min_score}
    &\underset{\boldsymbol{\theta}^{[i]}}{\max}~score_i\\ \nonumber
    &\text{s.t.} ~~ \boldsymbol{\theta}^{[i]}=[\theta^{[i]}_1,\theta^{[i]}_2,\ldots,\theta^{[i]}_{M}], ~~ \theta^{[i]}_{m}\in \phi_N \quad~ \text{for}~ 1\leq m \leq M, ~ 1\leq i \leq K.
\end{align}
Here, we use the same strategy as in Section~\ref{sub_subsect_optim_central_RIS} to maximize \eqref{eq:opt_max_min_score} since the filled function can be applied to a general unconstrained optimization problem.

Notice that it is possible to use two other methods to define $score_i$: (1) SNR at $i^{\mathrm{th}}$ receiver ($\text{SNR}_i$); and (2) signal-to-interference-ratio from ${\sf Tx}_i$ (SIR-${\sf Tx}_i$) by removing noise from the denominator of \eqref{eq:score_i}. %{\color{red} do you simply mean max $SNR_i$? then say that.} {\color{red} how is this different from (17)? just noise? If not, (17) really needs some explanation.}
In Fig.~\ref{Fig:sinr_sir_snr},  %{\color{red}Thuan: we must elaborate differences among (a), (b), (c) and give reasonable explanations.}
we compare the performance of these two alternatives with $score_i$ in \eqref{eq:score_i} utilizing different transmit powers. It depicts that $score_i$ consistently outperforms the other two ways %{\color{blue}
since it includes the impact of desired and interference signals from ${\sf Tx}_i$ as well as noise. In addition, Fig.~\ref{Fig:sinr_sir_snr} shows that $\text{SNR}_i$ performs better than SIR-${\sf Tx}_i$ when $P_i$ is small because the desired and interference signals are weak, while SIR-${\sf Tx}_i$ does better than $\text{SNR}_i$ at high $P_i$ values due to the strong interference signals, and the difference between the curves using $score_i$ and SIR-${\sf Tx}_i$ decreases as $P_i$ increases.

\subsubsection{Lower bound on the minimum number of elements at $\text{RIS}_i$}
\label{sub_subsect_lower_bound_dist_RIS}
By considering the same symmetric setting as mentioned in Section~\ref{sub_subsect_lower_bound_central_RIS}, we show a lower bound on the minimum number of RIS elements that ensures achieving a given value of {\it $\text{score}_i$}, as $\Tilde{score}$, which is calculated for $10 < M < 512$ as follows:
 \begin{align}
    M>\underset{a}{\min}\Big\{(K-1)\log_N\Big[\frac{\Tilde{score}\frac{\pi}{2}(K-1)(\sigma_{h_d}^2+512\nu^{\prime})}{(\sigma_{h_d}^2+10\nu^{\prime})\Big[Q^{-1}\big(\frac{1}{2N^{a/2}}\big)\Big]^2-\frac{\sigma^2}{P}\Tilde{score}}\Big]+a\Big\},
\end{align}
where $a$ is a trade-off between signal improvement from ${\sf Tx}_i$ at desired receiver and suppressing the interference signals from ${\sf Tx}_i$ at undesired receivers.
The details are presented in Section~\ref{Section:min_M}.

==> sections/Section5_min_M_v1.tex <==
In this section, we derive a lower bound on minimum number of elements in RIS to guarantee $\text{SINR}_i$ is large enough for successful decoding at ${\sf Rx}_i$. In particular, we consider a symmetric setting where all transmitters have the same transmit power $P_i=P, i=\{1,2,\ldots,K\}$ and receivers are located at the same distance from transmitters. 

Despite RIS elements should be obtained based on the channel coefficients, here to find a lower bound on $M$, we assume that different phase configurations $\boldsymbol{\theta}$ are independent from the channels and selected randomly with uniform distribution. Then, we use two following lemmas to explain our analysis.
\begin{lemma}
\label{lemma:avg_variance}
If $h_{ji}$ represents the channel coefficient between ${\sf Tx}_j$ and ${\sf Rx}_i$, $\mathbf{G}_i^{[1]}$ denotes the channel vector between ${\sf Tx}_i$ and RIS, and $\mathbf{G}_i^{[2]}$ shows the channel vector between RIS and ${\sf Rx}_i$ whose elements are independent and identically distributed (i.i.d.) random variables with mean $0$, $m_{g^{[1]}}$, and $0$, and variance $\sigma^2_h$, $\sigma_{g^{[1]}}^2$, and $\sigma_{g^{[2]}}^2$, respectively. Then, for a given RIS configuration $\mathbf{\Theta}$ where all elements are independent and drawn randomly from $\{0,\frac{2\pi}{N},\frac{4\pi}{N},\ldots,\frac{2\pi(N-1)}{N}\}$, we have
\begin{align}
    \label{eq:lemma_avg_variance}
    \nu=\text{var}(h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]})=\sigma^2_h+M\big[\sigma_{g^{[1]}}^2\sigma_{g^{[2]}}^2+\sigma_{g^{[2]}}^2(m_{g^{[1]}})^2\big].
\end{align}
%where $\text{var}(h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]})$ describes the variance of $h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}$.
\end{lemma}
\begin{proof}
We have 
\begin{align}
\label{eq:proof_variance_lemma}
    \nu&=\text{var}(h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]})=\text{var}(h_{ji}+\sum_{m=1}^Mg_{jm}^{[1]}e^{j\theta_m}g_{mi}^{[2]})\overset{(a)}{=}\text{var}(h_{ji})+\sum_{m=1}^M\text{var}(g_{jm}^{[1]}e^{j\theta_m}g_{mi}^{[2]})\\ \nonumber
    &\overset{(b)}{=}\sigma_h^2+\sum_{m=1}^M\Big(\sigma_{g^{[1]}}^2+(m_{g^{[1]}})^2\Big)\Big(\underbrace{\text{var}\{e^{j\theta_m}\}}_{1}+\underbrace{[\mathbb{E}\{e^{j\theta_m}\}]^2}_{=0}\Big)\sigma_{g^{[2]}}^2-\Big(\underbrace{[m_{g^{[1]}}]^2[\mathbb{E}\{e^{j\theta_m}\}]^2[\mathbb{E}\{g_{mi}^{[2]}\}]^2}_{=0}\Big)\\ \nonumber &=\sigma^2_h+M\big[\sigma_{g^{[1]}}^2\sigma_{g^{[2]}}^2+\sigma_{g^{[2]}}^2(m_{g^{[1]}})^2\big],
\end{align}
where $g_{jm}^{[1]}$ and $g_{mi}^{[2]}$ represent the $\text{m}^{\text{th}}$ element of $\mathbf{G}_j^{[1]}$ and $\mathbf{G}_i^{[2]}$, respectively, $(a)$ holds because $g_{jm}^{[1]}$, $e^{j\theta_m}$, and $g_{mi}^{[2]}$ are independent, and $(b)$ follows the rule of the variance of the product of three independent variables. As a result, \eqref{eq:proof_variance_lemma} completes the proof.
\end{proof}

\begin{lemma}
\label{lemma:avg_mean}
Using the assumptions in Lemma~\ref{lemma:avg_variance}, we have
\begin{align}
    \label{eq:lemma_avg_mean}
    \mu=\text{mean}(h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]})=0.
\end{align}
%where $\text{mean}(h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]})$ shows the mean of $h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}$.
\end{lemma}

\begin{proof}
Since different phase configurations $\boldsymbol{\theta}$ are chosen randomly based on uniform distribution, we have
\begin{align}
    \mu&=\text{mean}(h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]})=\text{mean}(h_{ji}+\sum_{m=1}^Mg_{jm}^{[1]}e^{j\theta_m}g_{mi}^{[2]})=\text{mean}(h_{ji})+\sum_{m=1}^M\text{mean}(g_{jm}^{[1]}g_{mi}^{[2]}e^{j\theta_m}) \\ \nonumber
    &\overset{(a)}{=}\underbrace{\mathbb{E}\{h_{ji}\}}_{=0}+\sum_{m=1}^M m_{g^{[1]}}\underbrace{\mathbb{E}\{g_{mi}^{[2]}\}}_{=0}\underbrace{\mathbb{E}(e^{j\theta_m})}_{=0}=0.
\end{align}
where $(a)$ is true because $g_{jm}^{[1]}$, $e^{j\theta_m}$, and $g_{mi}^{[2]}$ are independent, and this completes the proof.
\end{proof}

Moreover, we use a Monte Carlo simulation as Fig.~\ref{Fig:monte_carlo} to show that $h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}$ is distributed as a zero-mean Gaussian distribution with variance $\nu$.

\begin{figure}[ht]
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=5, width=0.6\linewidth, draft=false]{images/gaussian_distrb.png}
  \caption{\it The Monte Carlo simulation.}\label{Fig:monte_carlo}
\end{figure}

We note that the following lemma plays an important role in our descriptions. Here, we have
\begin{lemma}
\label{lemma:approx_prob}
For any $\delta>0$, 
\begin{align}
\label{eq:prob_less_delta}
    \Pr\Big(\Big|h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\Big|<\delta\Big|\mathbf{\Theta}\Big)&>\Pr\Big(\Big|Re\{h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta}\Big)\Pr\Big(\Big|Im\{h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta}\Big) \\ \nonumber
    &\approx(\frac{\sqrt{2}\delta}{\sqrt{\pi \nu}})^2, j\in\{1,2,\ldots,K\}, j\neq i.
\end{align}
\end{lemma}

\begin{proof}
For a given $\mathbf{\Theta}$, we have
\begin{align}
\label{eq:intersect_real_imag}
    \Pr\Big(\Big|h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\Big|<\delta\Big|\mathbf{\Theta}\Big)&>\Pr\Big(\Big|Re\{h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta} \bigcap \Big|Im\{h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta}\Big).
\end{align}
We define $X\triangleq Re\{h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\}$ and $Y\triangleq Im\{h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\}$ to make the proof easier to understand. Then, to simplify \eqref{eq:intersect_real_imag}, we need to show that $|X|$ and $|Y|$ are independent. We note that the independence of $X$ and $Y$ leads to the independence of $|X|$ and $|Y|$ since applying any function to two independent variables does not change the independence property. Thus, we remove the absolute function from the rest of the proof. Furthermore, from Lemma~\ref{lemma:avg_variance}, we know that $X$ and $Y$ are two random variables, which are distributed based on zero-mean Gaussian distribution. Therefore, $X$ and $Y$ are independent if they are uncorrelated (i.e., $Cov(X,Y)=0$). Hence, to show $Cov(X,Y)$, we write
\begin{align}
    Cov(X,Y)=\mathbb{E}(XY)-\mathbb{E}(X)\mathbb{E}(Y)\overset{(a)}{=}\mathbb{E}(XY),
\end{align}
where $(a)$ holds because $X$ and $Y$ are zero-mean random variables. Then, we have
\begin{align}
\label{eq:e_xy_ini}
    \mathbb{E}(XY)=\mathbb{E}\Big\{Re\big\{h_{ji}+\sum_{m=1}^Mg_{jm}^{[1]}e^{j\theta_m}g_{mi}^{[2]}\big\}Im\big\{h_{ji}+\sum_{m^{\prime}=1}^Mg_{jm^{\prime}}^{[1]}e^{j\theta_{m^{\prime}}}g_{m^{\prime}i}^{[2]}\big\}\Big\}.
\end{align}
We use superscript $R$ and $I$ to denote the real and imaginary parts of the channels ($h_{ji},g_{jm}^{[1]}$ and $g_{mi}^{[2]}$) and rewrite \eqref{eq:e_xy_ini} as
\begin{align}
\label{eq:e_xy_first_zeros}
    \mathbb{E}(XY)&=\mathbb{E}\Big\{\Big[h^R_{ji}+\sum_{m=1}^M(g_{jm}^{[1]R}g_{mi}^{[2]R}-g_{jm}^{[1]I}g_{mi}^{[2]I})cos \theta_m-(g_{jm}^{[1]R}g_{mi}^{[2]I}+g_{jm}^{[1]I}g_{mi}^{[2]R})sin \theta_m\Big] \\ \nonumber &\times \Big[h^I_{ji}+\sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]R}-g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]I})sin \theta_{m^{\prime}}+(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]I}+g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]R})cos \theta_{m^{\prime}}\Big]\Big\}\\ \nonumber
    &\overset{(b)}{=}\underbrace{\mathbb{E}\{h^R_{ji}h^I_{ji}\}}_{=0}+\underbrace{\mathbb{E}\Big\{h^I_{ji}\Big[\sum_{m=1}^M(g_{jm}^{[1]R}g_{mi}^{[2]R}-g_{jm}^{[1]I}g_{mi}^{[2]I})cos \theta_m-(g_{jm}^{[1]R}g_{mi}^{[2]I}+g_{jm}^{[1]I}g_{mi}^{[2]R})sin \theta_m\Big]\Big\}}_{=0}\\ \nonumber
    &+\underbrace{\mathbb{E}\Big\{h^R_{ji}\Big[\sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]R}-g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]I})sin \theta_{m^{\prime}}+(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]I}+g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]R})cos \theta_{m^{\prime}}\Big]\Big\}}_{=0} \\ \nonumber
    &+\mathbb{E}\Big\{\Big[\sum_{m=1}^M(g_{jm}^{[1]R}g_{mi}^{[2]R}-g_{jm}^{[1]I}g_{mi}^{[2]I})cos \theta_m-(g_{jm}^{[1]R}g_{mi}^{[2]I}+g_{jm}^{[1]I}g_{mi}^{[2]R})sin \theta_m\Big] \\ \nonumber 
    &\times \Big[\sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]R}-g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]I})sin \theta_{m^{\prime}}+(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]I}+g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]R})cos \theta_{m^{\prime}}\Big]\Big\},
\end{align}
where $(b)$ is correct since $h^R_{ji}$, $h^I_{ji}$, $g_{jm}^{[1]R},g_{mi}^{[2]R}$, $g_{jm}^{[1]I},g_{mi}^{[2]I}$,$g_{jm^{\prime}}^{[1]R},g_{m^{\prime}i}^{[2]R}$, $g_{jm^{\prime}}^{[1]I}$, and $g_{m^{\prime}i}^{[2]I}$ are independent and $\mathbb{E}\{h^R_{ji}\}=\mathbb{E}\{h^I_{ji}\}=0$. Then, we derive $\mathbb{E}(XY)$ through two cases: (i) $m=m^{\prime}$; (ii) $m\neq m^{\prime}$. Below, we describe these cases.

$\bullet~\mathbf{m=m^{\prime}:}$ In this case, since $m=m^{\prime}$ and $\mathbb{E}(XY)$ should hold for any given value of $M$, we consider $M=1$ and simplify \eqref{eq:e_xy_first_zeros} as
\begin{align}
\label{eq:m_m_complete}
    &\mathbb{E}(XY)\\ \nonumber
    &=\mathbb{E}\Big\{\Big[(g_{jm}^{[1]R}g_{mi}^{[2]R}-g_{jm}^{[1]I}g_{mi}^{[2]I})cos \theta_m-(g_{jm}^{[1]R}g_{mi}^{[2]I}+g_{jm}^{[1]I}g_{mi}^{[2]R})sin \theta_m\Big] \\ \nonumber 
    &\times \Big[(g_{jm}^{[1]R}g_{m^i}^{[2]R}-g_{jm}^{[1]I}g_{mi}^{[2]I})sin \theta_{m}+(g_{jm}^{[1]R}g_{mi}^{[2]I}+g_{jm}^{[1]I}g_{mi}^{[2]R})cos \theta_{m}\Big]\Big\}\\ \nonumber
    &= \mathbb{E}\Big\{\Big[(g_{jm}^{[1]R}g_{mi}^{[2]R}-g_{jm}^{[1]I}g_{mi}^{[2]I})(g_{jm}^{[1]R}g_{mi}^{[2]I}+g_{jm}^{[1]I}g_{mi}^{[2]R})(cos^2\theta_m-sin^2\theta_m)\Big] \\ \nonumber 
    &+\frac{1}{2}\mathbb{E}\Big\{\Big[(g_{jm}^{[1]R}g_{mi}^{[2]R}-g_{jm}^{[1]I}g_{mi}^{[2]I})^2-(g_{jm}^{[1]R}g_{mi}^{[2]I}+g_{jm}^{[1]I}g_{mi}^{[2]R})^2\Big]sin2\theta_m\Big\}\\ \nonumber
    &=\mathbb{E}\Big\{\Big[(g_{jm}^{[1]R})^2-(g_{jm}^{[1]I})^2\Big]g_{mi}^{[2]R}g_{mi}^{[2]I}cos2\theta_m+\Big[(g_{mi}^{[2]R})^2-(g_{mi}^{[2]I})^2\Big]g_{jm}^{[1]R}g_{jm}^{[1]I}cos2\theta_m\Big\}\\ \nonumber
    &+\frac{1}{2}\mathbb{E}\Big\{\Big[(g_{jm}^{[1]R}g_{mi}^{[2]R})^2+(g_{jm}^{[1]I}g_{mi}^{[2]I})^2-(g_{jm}^{[1]R}g_{mi}^{[2]I})^2-(g_{jm}^{[1]I}g_{mi}^{[2]R})^2-4g_{jm}^{[1]R}g_{mi}^{[2]R}g_{jm}^{[1]I}g_{mi}^{[2]I}\Big]sin2\theta_m\Big\}\\ \nonumber
    &\overset{(c)}{=}\mathbb{E}\Big\{\Big[(g_{jm}^{[1]R})^2-(g_{jm}^{[1]I})^2\Big]g_{mi}^{[2]R}g_{mi}^{[2]I}cos2\theta_m\Big\}+\mathbb{E}\Big\{\Big[(g_{mi}^{[2]R})^2-(g_{mi}^{[2]I})^2\Big]g_{jm}^{[1]R}g_{jm}^{[1]I}cos2\theta_m\Big\} \\ \nonumber
    &+\frac{1}{2}\Big(\mathbb{E}\Big\{(g_{jm}^{[1]R})^2\big[(g_{mi}^{[2]R})^2-(g_{mi}^{[2]I})^2\big]\Big\}+\mathbb{E}\Big\{(g_{jm}^{[1]I})^2\big[(g_{mi}^{[2]I})^2-(g_{mi}^{[2]R})^2\big]\Big\}-4\mathbb{E}\Big\{g_{jm}^{[1]R}g_{mi}^{[2]R}g_{jm}^{[1]I}g_{mi}^{[2]I}\Big\}\Big)sin2\theta_m\\ \nonumber
    &\overset{(d)}{=}\mathbb{E}\Big\{\Big[(g_{jm}^{[1]R})^2-(g_{jm}^{[1]I})^2\Big]\Big\}\mathbb{E}\Big\{g_{mi}^{[2]R}g_{mi}^{[2]I}\Big\}cos2\theta_m+\mathbb{E}\Big\{\Big[(g_{mi}^{[2]R})^2-(g_{mi}^{[2]I})^2\Big]\Big\}\mathbb{E}\Big\{g_{jm}^{[1]R}g_{jm}^{[1]I}\Big\}cos2\theta_m \\ \nonumber
    &+\frac{1}{2}\Big(\mathbb{E}\Big\{(g_{jm}^{[1]R})^2\Big\}\mathbb{E}\Big\{\big[(g_{mi}^{[2]R})^2-(g_{mi}^{[2]I})^2\big]\Big\}+\mathbb{E}\Big\{(g_{jm}^{[1]I})^2\Big\}\mathbb{E}\Big\{\big[(g_{mi}^{[2]I})^2-(g_{mi}^{[2]R})^2\big]\Big\}-4\mathbb{E}\Big\{g_{jm}^{[1]R}g_{jm}^{[1]I}\Big\}\mathbb{E}\Big\{g_{mi}^{[2]R}g_{mi}^{[2]I}\Big\}\Big)sin2\theta_m\\ \nonumber
    &\overset{(e)}{=}\underbrace{\mathbb{E}\Big\{\Big[(g_{jm}^{[1]R})^2-(g_{jm}^{[1]I})^2\Big]\Big\}}_{=0}\mathbb{E}\Big\{g_{mi}^{[2]R}g_{mi}^{[2]I}\Big\}cos2\theta_m+\underbrace{\mathbb{E}\Big\{\Big[(g_{mi}^{[2]R})^2-(g_{mi}^{[2]I})^2\Big]\Big\}}_{=0}\mathbb{E}\Big\{g_{jm}^{[1]R}g_{jm}^{[1]I}\Big\}cos2\theta_m \\ \nonumber
    &+\frac{1}{2}\Big(\mathbb{E}\Big\{(g_{jm}^{[1]R})^2\Big\}\underbrace{\mathbb{E}\Big\{\big[(g_{mi}^{[2]R})^2-(g_{mi}^{[2]I})^2\big]\Big\}}_{=0}+\mathbb{E}\Big\{(g_{jm}^{[1]I})^2\Big\}\underbrace{\mathbb{E}\Big\{\big[(g_{mi}^{[2]I})^2-(g_{mi}^{[2]R})^2\big]\Big\}}_{=0}-4\mathbb{E}\Big\{g_{jm}^{[1]R}g_{jm}^{[1]I}\Big\}\underbrace{\mathbb{E}\Big\{g_{mi}^{[2]R}g_{mi}^{[2]I}\Big\}}_{=0}\Big)sin2\theta_m\\ \nonumber
    &=0,
\end{align}
where $(c)$ happens since the expected value operator is linear, and $(d)$ and $(e)$ are true because (i) the real and imaginary parts of the channels are independent; (ii) $\mathbb{E}\Big\{(g_{mi}^{[2]I})^2\Big\}=\mathbb{E}\Big\{(g_{mi}^{[2]R})^2\Big\}$; (iii) $\mathbb{E}\Big\{g_{mi}^{[2]R}\Big\}=\mathbb{E}\Big\{g_{mi}^{[2]I}\Big\}=0$.
$\bullet~\mathbf{m\neq m^{\prime}}:$ In this case, we have
\begin{align}
\label{eq:four_terms}
    \mathbb{E}(XY)&=\mathbb{E}\Big\{\Big[\sum_{m=1}^M(g_{jm}^{[1]R}g_{mi}^{[2]R}-g_{jm}^{[1]I}g_{mi}^{[2]I})cos \theta_m-(g_{jm}^{[1]R}g_{mi}^{[2]I}+g_{jm}^{[1]I}g_{mi}^{[2]R})sin \theta_m\Big] \\ \nonumber 
    &\times \Big[\sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]R}-g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]I})sin \theta_{m^{\prime}}+(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]I}+g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]R})cos \theta_{m^{\prime}}\Big]\Big\}.
\end{align}

Then, we use the linear property of the expected value operator and break \eqref{eq:four_terms} into four terms as \eqref{eq:first_product}, \eqref{eq:second_product}, \eqref{eq:third_product}, and \eqref{eq:fourth_product}. Here are the details.
\begin{align}
\label{eq:first_product}
    &\mathbb{E}\Big\{\sum_{m=1}^M(g_{jm}^{[1]R}g_{mi}^{[2]R}-g_{jm}^{[1]I}g_{mi}^{[2]I})cos \theta_m\times \sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]R}-g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]I})sin \theta_{m^{\prime}}\Big\} \\ \nonumber
    &\overset{(f)}{=}\mathbb{E}\Big\{\sum_{m=1}^M(g_{jm}^{[1]R}g_{mi}^{[2]R})cos \theta_m \sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]R})sin \theta_{m^{\prime}}\Big\}-\mathbb{E}\Big\{\sum_{m=1}^M(g_{jm}^{[1]I}g_{mi}^{[2]I})cos \theta_m \sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]R})sin \theta_{m^{\prime}}\Big\} \\ \nonumber
    &+\mathbb{E}\Big\{\sum_{m=1}^M(g_{jm}^{[1]I}g_{mi}^{[2]I})cos \theta_m \sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]I})sin \theta_{m^{\prime}}\Big\}-\mathbb{E}\Big\{\sum_{m=1}^M(g_{jm}^{[1]R}g_{mi}^{[2]R})cos \theta_m \sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]I})sin \theta_{m^{\prime}}\Big\} \\ \nonumber
    &\overset{(g)}{=}\mathbb{E}\Big\{\sum_{m=1}^M(g_{jm}^{[1]R}g_{mi}^{[2]R})cos \theta_m\Big\} \mathbb{E}\Big\{\sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]R})sin \theta_{m^{\prime}}\Big\}-\mathbb{E}\Big\{\sum_{m=1}^M(g_{jm}^{[1]I}g_{mi}^{[2]I})cos \theta_m\Big\} \mathbb{E}\Big\{\sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]R})sin \theta_{m^{\prime}}\Big\} \\ \nonumber
    &+\mathbb{E}\Big\{\sum_{m=1}^M(g_{jm}^{[1]I}g_{mi}^{[2]I})cos \theta_m\Big\} \mathbb{E}\Big\{\sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]I})sin \theta_{m^{\prime}}\Big\}-\mathbb{E}\Big\{\sum_{m=1}^M(g_{jm}^{[1]R}g_{mi}^{[2]R})cos \theta_m \Big\}\mathbb{E}\Big\{\sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]I})sin \theta_{m^{\prime}}\Big\}\\ \nonumber
    &\overset{(h)}{=}\sum_{m=1}^M\underbrace{\mathbb{E}\{g_{mi}^{[2]R}\}}_{=0}\mathbb{E}\{g_{jm}^{[1]R}cos \theta_m\} \sum_{m^{\prime}=1}^M\underbrace{\mathbb{E}\{g_{m^{\prime}i}^{[2]R}\}}_{=0}\mathbb{E}\{g_{jm^{\prime}}^{[1]R}sin \theta_{m^{\prime}}\}-\sum_{m=1}^M\underbrace{\mathbb{E}\{g_{mi}^{[2]I}\}}_{=0}\mathbb{E}\{g_{jm}^{[1]I}cos \theta_m\} \sum_{m^{\prime}=1}^M\underbrace{\mathbb{E}\{g_{m^{\prime}i}^{[2]R}\}}_{=0}\mathbb{E}\{g_{jm^{\prime}}^{[1]R}sin \theta_{m^{\prime}}\} \\ \nonumber
    &+\sum_{m=1}^M\underbrace{\mathbb{E}\{g_{mi}^{[2]I}\}}_{=0}\mathbb{E}\{g_{jm}^{[1]I}cos \theta_m\} \sum_{m^{\prime}=1}^M\underbrace{\mathbb{E}\{g_{m^{\prime}i}^{[2]I}\}}_{=0}\mathbb{E}\{g_{jm^{\prime}}^{[1]I}sin \theta_{m^{\prime}}\}-\sum_{m=1}^M\underbrace{\mathbb{E}\{g_{mi}^{[2]R}\}}_{=0}\mathbb{E}\{g_{jm}^{[1]R}cos \theta_m \}\sum_{m^{\prime}=1}^M\underbrace{\mathbb{E}\{g_{m^{\prime}i}^{[2]I}\}}_{=0}\mathbb{E}\{g_{jm^{\prime}}^{[1]I}sin \theta_{m^{\prime}}\}\\ \nonumber
    &=0,
\end{align}
where $(f)$ follows the linear property of the expected value operator, and $(g)$ and $(h)$ are true because $h^R_{ji}$, $h^I_{ji}$, $g_{jm}^{[1]R},g_{mi}^{[2]R}$, $g_{jm}^{[1]I},g_{mi}^{[2]I}$,$g_{jm^{\prime}}^{[1]R},g_{m^{\prime}i}^{[2]R}$, $g_{jm^{\prime}}^{[1]I}$, and $g_{m^{\prime}i}^{[2]I}$ are independent.
Similar to \eqref{eq:first_product}, we can show that
\begin{align}
\label{eq:second_product}
    \mathbb{E}\Big\{\sum_{m=1}^M(g_{jm}^{[1]R}g_{mi}^{[2]R}-g_{jm}^{[1]I}g_{mi}^{[2]I})cos \theta_m\times \sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]I}-g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]R})cos \theta_{m^{\prime}}\Big\}=0,
\end{align}
\begin{align}
\label{eq:third_product}
    \mathbb{E}\Big\{\sum_{m=1}^M(g_{jm}^{[1]R}g_{mi}^{[2]I}-g_{jm}^{[1]I}g_{mi}^{[2]R})sin \theta_m\times \sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]R}-g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]I})sin \theta_{m^{\prime}}\Big\}=0,
\end{align}

\begin{align}
\label{eq:fourth_product}
    \mathbb{E}\Big\{\sum_{m=1}^M(g_{jm}^{[1]R}g_{mi}^{[2]I}-g_{jm}^{[1]I}g_{mi}^{[2]R})sin \theta_m\times \sum_{m^{\prime}=1}^M(g_{jm^{\prime}}^{[1]R}g_{m^{\prime}i}^{[2]I}-g_{jm^{\prime}}^{[1]I}g_{m^{\prime}i}^{[2]R})sin \theta_{m^{\prime}}\Big\}=0.
\end{align}

Therefore, using \eqref{eq:m_m_complete}, \eqref{eq:first_product}, \eqref{eq:second_product}, \eqref{eq:third_product}, and \eqref{eq:fourth_product} prove that $\mathbb{E}\{XY\}=0$, and this means that $X$ and $Y$ are independent.

As a result, we simplify \eqref{eq:intersect_real_imag} as 
\begin{align}
    \Pr\Big(\Big|h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\Big|<\delta\Big|\mathbf{\Theta}\Big)&>\Pr\Big(\Big|Re\{h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta}\Big)\Pr\Big(\Big|Im\{h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta}\Big), \\ \nonumber & j\in\{1,2,\ldots,K\}, j\neq i.
\end{align}
Since $Re\{h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\}$ is a zero-mean Gaussian random variable, we have
\begin{align}
    \Pr\Big(\Big|Re\{h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta}\Big)&=\int_{-\frac{\delta}{\sqrt{2}}}^{\frac{\delta}{\sqrt{2}}}\frac{1}{\sqrt{\pi \nu}}e^{\frac{-r^2}{\nu}}dr \\ \nonumber
    &\overset{(q)}{\approx}\int_{-\frac{\delta}{\sqrt{2}}}^{\frac{\delta}{\sqrt{2}}}\frac{1}{\sqrt{\pi \nu}}\Big[1-\frac{r^2}{\nu}+O (\frac{r^4}{\nu^2})\Big]dr\\ \nonumber
    &=\frac{1}{\sqrt{\pi \nu}} \Big[\sqrt{2}\delta-\frac{\delta^3}{3\sqrt{2}\nu}+O(\frac{r^5}{\nu^2}) \Big]\\ \nonumber
    &\overset{(\ell)}{\approx}(\frac{\sqrt{2}\delta}{\sqrt{\pi \nu}}), ~~ j\in\{1,2,\ldots,K\}, j\neq i,
\end{align}
where $(q)$ applies based on approximation from the Taylor expansion of $e^{\frac{-r^2}{\nu}}$, and $(\ell)$ holds since our goal is to have small $\delta$; therefore, we ignore the high orders of $\frac{r}{\nu}$.

Similarly, we obtain
\begin{align}
    \Pr\Big(\Big|Im\{h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\}\Big|<\frac{\delta}{\sqrt{2}}\Big|\mathbf{\Theta}\Big)\approx(\frac{\sqrt{2}\delta}{\sqrt{\pi \nu}}), ~~ j\in\{1,2,\ldots,K\}, j\neq i.
\end{align}

Hence, using (24) and (25) leads to
\begin{align}
    \Pr\Big(\Big|h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}\Big|<\delta\Big|\mathbf{\Theta}\Big)&>(\frac{\sqrt{2}\delta}{\sqrt{\pi \nu}})^2, j\in\{1,2,\ldots,K\}, j\neq i,
\end{align}
which completes the proof.
\end{proof}
We know the above condition should happens for all interfering signals at ${\sf Rx}_i$. Therefore, we define $\Pr(I<\delta)$ as
\begin{align}
    \Pr(I<\delta)\triangleq \Pr(|h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}|<\delta), \quad \text{for all}~j\in \{1,2,\ldots,K\}, j\neq i.
\end{align}

Furthermore, we assume all channels are i.i.d. across time and users. Hence,
\begin{align}
\label{eq:approx_prob_all}
    \Pr(I<\delta)=\prod_{j\in K, j\neq i}\Pr(|h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}|<\delta)>(\frac{2\delta}{\sqrt{2\pi \nu}})^{2(K-1)}.
\end{align}


Then, to simplify the description of $\nu$, we define $\nu^{\prime}$ as 
\begin{align}
    \nu^{\prime}\triangleq \big[\sigma_{g^{[1]}}^2\sigma_{g^{[1]}}^2+\sigma_{g^{[2]}}^2(m_{g^{[1]}})^2\big].
\end{align}

Finally, we use the following lemma to derive a lower bound of minimum number of element in RIS.

\begin{lemma}
\label{lemma:Min_M_RIS}
The achievable a given signal-to-interference-plus-noise ratio, $\tilde{\text{SINR}}$, per user almost surely given the minimum number of element in RIS as:
\begin{align}
    M>\frac{1}{\nu^{\prime}}\Big[\frac{[\sigma^2+P(K-1)\frac{\pi}{2}(\sigma_h^2+512\nu^{\prime})N^{(\frac{-9}{K(K-1)})}]\Tilde{\text{SINR}}}{P}-\sigma^2_h\Big].
\end{align}
\end{lemma}

\begin{proof}
From \eqref{eq:approx_prob_all}, we know $\Pr(I<\delta))>(\frac{2\delta}{\sqrt{2\pi \nu}})^{2(K-1)}$. In addition, we have $N^{M-1}$ possible combination for RIS elements and these $N^{M-1}$ are available for all $K$ users, which means we only access to $N^{M-1}$ RIS configurations to obtain a given $\tilde{\text{SINR}}$ for all users. Thus, to get a given $\tilde{\text{SINR}}$ with high probability at all receivers, we need
\begin{align}
\label{eq_high_prob}
    N^{M-1}(\frac{2\delta}{\sqrt{2 \pi (\sigma_h^2+M\nu^{\prime})}})^{2K(K-1)}>1.
\end{align}

By taking $\log_N$ from both sides of \eqref{eq_high_prob}, we find
\begin{align}
\label{eq_first_eq_M}
    M>2K(K-1)\log_N\Big(\frac{\sqrt{\pi (\sigma_h^2+M\nu^{\prime})}}{\sqrt{2}\delta}\Big)+1.
\end{align}

Due to the practical limits, we assume $10 \leq M\leq 512$ and relax the right-hand side of \eqref{eq_first_eq_M}. This way, we have
\begin{align}
\label{eq_2nd_eq_M}
    M>2K(K-1)\log_N\Big(\frac{\sqrt{\pi (\sigma_h^2+512\nu^{\prime})}}{\sqrt{2}\delta}\Big)+1.
\end{align}

We know the number of RIS elements is an integer number. Thus, $M=\ceil*{2K(K-1)\log_N\Big(\frac{\sqrt{\pi (\sigma_h^2+512\nu^{\prime})}}{\sqrt{2}\delta}\Big)+1}$ represent the minimum number of elements at RIS that leads to 
\begin{align}
\label{eq:delta_value}
    \delta<N^{-(\frac{M-1}{2K(K-1)})}\sqrt{\frac{\pi}{2}(\sigma_h^2+512\nu^{\prime})}.
\end{align}

Here, we define $\tilde{\text{SINR}}$ as a lower bound of SINR at ${\sf Rx}_i$. Moreover, as we discussed in Lemma~\ref{lemma:avg_variance} and \ref{lemma:avg_mean},  $h_{ji}+\mathbf{G}_j^{[1]}\mathbf{\Theta}\mathbf{G}_i^{[2]}$ follows a complex zero-mean Gaussian distribution with variance $\nu$. As a result, we have
\begin{align}
\label{eq:bar_SINR}
\Tilde{\text{SINR}}&=\int_{-\infty}^{+\infty}\frac{P\delta^{\prime 2}}{\sigma^2+P(K-1)\delta^2}f_i(\delta^{\prime})d\delta^{\prime},\\ \nonumber
&=\frac{P}{\sigma^2+P(K-1)\delta^2}\int_{-\infty}^{+\infty}\delta^{\prime 2}f_i(\delta^{\prime})d\delta^{\prime}\overset{(a)}{=}\frac{P \nu}{\sigma^2+P(K-1)\delta^2},
\end{align}
where $f_i(\delta^{\prime})$ is a complex zero-mean Gaussian distribution with variance $\nu$ and $(a)$ is correct because  $\int_{-\infty}^{+\infty}\delta^{\prime 2}f_i(\delta^{\prime})d\delta^{\prime}=\nu$. Then, using \eqref{eq:delta_value}, and \eqref{eq:bar_SINR}, we have:
\begin{align}
    \label{eq:final_bar_SINR}
    \Tilde{\text{SINR}}&>\frac{P(\sigma_h^2+M\nu^{\prime})}{\sigma^2+P(K-1)\frac{\pi}{2}(\sigma_h^2+512\nu^{\prime})N^{-(\frac{(M-1)}{K(K-1)})}}
\end{align}
By considering $10\leq M\leq 512$, we have
\begin{align}
    M>\frac{1}{\nu^{\prime}}\Big[\frac{[\sigma^2+P(K-1)\frac{\pi}{2}(\sigma_h^2+512\nu^{\prime})N^{(\frac{-9}{K(K-1)})}]\Tilde{\text{SINR}}}{P}-\sigma^2_h\Big],
\end{align}
which completes the proof.
\end{proof}

==> sections/Section6_extension_to_K_RIS_network.tex <==
In this section, we focus on a network with $K$ distributed RISs and show a lower bound on $M$ that guarantees achieving a given value of $score_i$ as $\Tilde{score}$. To do this, assume a symmetric scenario as Section~\ref{Section:min_M} where all RISs have the same number of elements. Then, we use the following Lemma.

\begin{lemma}
\label{lemma:Min_M_score}
The achievable a given $score_i$, $\Tilde{score}$, per user almost surely given the minimum number of elements in $\text{RIS}_i$ as:
 \begin{align}
    M>\underset{a}{\min}\Big\{(K-1)\log_N\Big[\frac{(\sigma_{h_d}^2+10\nu^{\prime})\Big[Q^{-1}\big(\frac{1}{2N^{a/2}}\big)\Big]^2-\frac{\sigma^2}{P}\Tilde{score}}{\Tilde{score}\frac{\pi}{2}(K-1)(\sigma_{h_d}^2+512\nu^{\prime})}\Big]+a\Big\},
\end{align}
\end{lemma}

\begin{proof}
We define $\Pr(I_{{\sf Tx}}<\delta)$ as
\begin{align}
\label{eq:Pr_I_Tx}
    \Pr(I_{{\sf Tx}}<\delta)\triangleq \Pr(|\textbf{g}^{[ij]}\mathbf{\Theta}^{[i]}\textbf{h}^{[ii]}+h_d^{[ij]}|<\delta) \quad \quad \text{for~all~} j\in \{1,2,\ldots,K\}, j\neq i.
\end{align}
Then, we rewrite \eqref{eq:Pr_I_Tx} as
\begin{align}
\label{eq:Pr_I_Tx_complete}
    \Pr(I_{{\sf Tx}}<\delta)\overset{(a)}{=}\prod_{j\in K, j\neq i}\Pr(|\textbf{g}^{[ij]}\mathbf{\Theta}^{[i]}\textbf{h}^{[ii]}+h_d^{[ij]}|<\delta)\overset{(b)}{>}(\frac{2\delta}{\sqrt{2\pi \nu}})^{2(K-1)},
\end{align}
where $(a)$ holds since we assume all channels are i.i.d. across time and users, and $(b)$ is correct using Lemma~\ref{lemma:approx_prob}. Similar to \eqref{eq:greater_Delta}, we can show that
\begin{align}
\label{eq:greater_Delta_Tx}
    \Pr\Big(\Big|\{\textbf{g}^{[ii]}\mathbf{\Theta}^{[i]}\textbf{h}^{[ii]}+h_d^{[ii]}\}\Big|>\frac{\Delta}{\sqrt{2}}\Big)>\big[2Q(\frac{\Delta}{\sqrt{\nu}})\big]^2.
\end{align}

Moreover, we have $N^{M}$ unique RIS configurations. As a result, to obtain a specific $\Tilde{score}$ with high probability at all receivers, we require
\begin{align}
    \label{eq:proof_min_M_Tx}
    N^{M}[2Q(\frac{\Delta}{\sqrt{\sigma^2_h+M\nu^{\prime}}})]^2(\frac{2\delta}{\sqrt{2 \pi(\sigma^2_h+M \nu^{\prime})}})^{2K(K-1)}>1.
\end{align}

Suppose
\begin{align}
\label{eq:assumption_delta_Tx}
    \delta=N^{\frac{-(M-a)}{2(K-1)}}\sqrt{\frac{\pi }{2}(\sigma_{h_d}^2+M^{+}\nu^{\prime})},
\end{align}
where $0 \leq a \leq M$ is a trade-off between improving the desired signal from ${\sf Tx}_i$ at ${\sf Rx}_i$ and suppressing the interference signals from ${\sf Tx}_i$ at ${\sf Rx}_j, j \neq i$. Then, we apply $\delta$ to \eqref{eq:proof_min_M_Tx} and get
\begin{align}
    N^a[2Q(\frac{\Delta}{\sqrt{\sigma_{h_d}^2+M\nu^{\prime}}})]^2(\frac{\sigma_{h_d}^2+M^{+}\nu^{\prime}}{\sigma_{h_d}^2+M\nu^{\prime}})^{(K-1)}>1.
\end{align}
Notice $(\frac{\sigma_{h_d}^2+M^{+}\nu^{\prime}}{\sigma_{h_d}^2+M\nu^{\prime}})^{(K-1)}>1$ since $M<{M^{+}}$. Hence, \eqref{eq:proof_min_M_Tx} holds true if
\begin{align}
    Q(\frac{\Delta}{\sqrt{\sigma_{h_d}^2+M\nu^{\prime}}})=\frac{1}{2N^{a/2}}.
\end{align}
Therefore, we have
\begin{align}
\label{eq:Delta_val_Tx}
    \Delta=\sqrt{\sigma_{h_d}^2+M\nu^{\prime}}\Big[Q^{-1}\big(\frac{1}{2N^{a/2}}\big)\Big].
\end{align}

Then, we conclude $\Tilde{score}$ at ${\sf Rx}_i$ as below:
\begin{align}
\label{eq:score_tild}
    \Tilde{score}&=\frac{\Big|\textbf{g}^{[ii]}\mathbf{\Theta}^{[i]}\textbf{h}^{[ii]}+h_d^{[ii]}\Big|^2}{\sigma^2+\sum_{j=1, j\neq i}^{K}\Big|\textbf{g}^{[ij]}\mathbf{\Theta}^{[i]}\textbf{h}^{[ii]}+h_d^{[ij]}\Big|^2}\overset{(c)}{>}\frac{P\Delta^2}{\sigma^2+P(K-1)\delta^2} \\ \nonumber
    &=\frac{(\sigma_{h_d}^2+M\nu^{\prime})\Big[Q^{-1}\big(\frac{1}{2N^{a/2}}\big)\Big]^2}{\frac{\sigma^2}{P}+\frac{\pi }{2}(K-1)N^{\frac{-(M-a)}{K(K-1)}}(\sigma_{h_d}^2+M^{+}\nu^{\prime})}\overset{(d)}{>}\frac{(\sigma_{h_d}^2+M^{-}\nu^{\prime})\Big[Q^{-1}\big(\frac{1}{2N^{a/2}}\big)\Big]^2}{\frac{\sigma^2}{P}+\frac{\pi }{2}(K-1)N^{\frac{-(M-a)}{K(K-1)}}(\sigma_{h_d}^2+M^{+}\nu^{\prime})},
\end{align}

where $(c)$ follows \eqref{eq:assumption_delta_Tx} and \eqref{eq:greater_Delta_Tx}, and $(d)$ is true because $M^{-}<M$. As shown in \eqref{eq:score_tild}, $\Tilde{score}$ depends on the value of $0\leq a \leq M$; thus, we find the best value of $a$ to maximize \eqref{eq:score_tild} numerically in Section~\ref{Section:Numerical}.


Finally, we take $\log_N$ from both sides of \eqref{eq:score_tild} and assume $10< M< 512$ and find the lower bound on $M$ as
 \begin{align}
    M>\underset{a}{\min}\Big\{(K-1)\log_N\Big[\frac{(\sigma_{h_d}^2+10\nu^{\prime})\Big[Q^{-1}\big(\frac{1}{2N^{a/2}}\big)\Big]^2-\frac{\sigma^2}{P}\Tilde{score}}{\Tilde{score}\frac{\pi}{2}(K-1)(\sigma_{h_d}^2+512\nu^{\prime})}\Big]+a\Big\},
\end{align}
which completes the proof.
\end{proof}

==> sections/abstract.tex <==
In this work, we study the benefits of utilizing reconfigurable-intelligent-surface (RIS) for spectrum efficiency in a single-input single-output (SISO) Internet of Things (IoT) network. We use low-bit phase shifters at RIS, resulting in a nonlinear integer programming (NLIP) problem. To control the RIS elements, we propose an optimization method to obtain an approximation of the optimal solution. To study the optimal placement of the RIS, we first use a centralized RIS, which needs imperfect global channel state information (CSI) to handle interference. We obtain the minimum number of RIS elements to fulfill a specific performance when the RIS moves from the transmitter toward the receiver. Then, we exploit $K$ distributed RISs, wherein one RIS is dedicated to each transmitter. We place each RIS close to its associated transmitter and assume that each transmitter only knows its imperfect outgoing channels to the receivers (local CSI at the transmitter). The simulation findings reveal that the distributed scenario outperforms the centralized case in terms of sum-rate and requires fewer RIS elements to achieve a given sum-rate. Finally, we provide a lower bound on the minimum number of RIS components required to achieve a particular performance. The results are validated using Monte-Carlo simulations.
